Exploiting Sparsity in Pruned Neural Networks to Optimize Large Model Training

Parallel training of neural networks at scale is challenging due to significant overheads arising from communication. Recently, deep learning researchers have developed a variety of pruning algorithms that are capable of pruning (i.e. setting to zero) 80-90% of the parameters in a neural network to yield sparse subnetworks that equal the accuracy of the unpruned parent network. In this work, we propose a novel approach that exploits these sparse subnetworks to optimize the memory utilization and communication in two popular algorithms for parallel deep learning namely -- data and inter-layer parallelism. We integrate our approach into AxoNN, a highly scalable framework for parallel deep learning that relies on data and inter-layer parallelism, and demonstrate the reduction in communication time and memory utilization. On 512 NVIDIA V100 GPUs, our optimizations reduce the memory consumption of a 2.7 billion parameter model by 74%, and the total communication time by 40%, thus providing an overall speedup of 34% over AxoNN, 32% over DeepSpeed-3D and 46% over Sputnik, a sparse matrix computation baseline.

==> memory.tex <==
We now derive the savings in GPU memory consumption that can be achieved by
using LTH-based pruning and \stod. For this analysis, we only consider the
model state memory i.e. the GPU memory required to store the half and full
precision parameters and gradients, and the optimizer states. We do not account
for the activation memory, for which the storage requirements depend on several
other factors in addition to the neural network architecture and the level of
sparsity induced by \stod.  We assume standard mixed precision
training~\cite{micikevicius2018mixed} with the Adam
optimizer~\cite{KingmaAdam2014}. As discussed in section \ref{sec:impl}, we
assume that a sparsified tensor is stored as a one-dimensional view in the
coordinate tensor format (COO).

\subsection{Terminology}

We use the following terms in deriving the equations below: 
\begin{itemize}
\item $\phi$ -- Total number of parameters in the neural network before pruning.
\item $\phi_{\mathrm{fc}}$ -- Total number of parameters before pruning that belong to FC layers.  
\item $\phi^\prime$ -- Total number of parameters in the neural network after pruning. 
\item $p$ -- Sparsity of a pruned parameter tensor.
\item $\vec{\theta}$ and $\nabla\vec{\theta}$ -- Full precision parameters and gradients.
\item $\vec{\theta}_{16}$ and $\nabla\vec{\theta}_{16}$ -- Half precision parameters and gradients.
\item $\vec{s}_{\mathrm{opt}}$ -- Adam optimizer states.
\item $M^{\mathrm{PG}}_{\mathrm{gpu}}$ -- Total GPU memory occupied by half-precision parameters and gradients ($\vec{\theta}_{16}$ and $\nabla\vec{\theta}_{16}$) after pruning.
\item $M_{\mathrm{gpu}}$ -- Total GPU memory occupied by $\vec{\theta}_{16}$, $\nabla\vec{\theta}_{16}$, $\vec{\theta}$, $\nabla\vec{\theta}$, and $\vec{s}_{\mathrm{opt}}$ after pruning.
\item $M^{\prime}_{\mathrm{gpu}}$ -- Same as above but with \axonn's memory optimizations also enabled in conjunction with LTH-based pruning.
\end{itemize}

\subsection{Memory Usage for Storing Model States}

We derive the memory usage for storing model states for two scenarios.  First,
when \stod is used as a stand-alone memory optimization and second, when it is
combined with \axonn's memory optimizations. Since we are pruning $p$ fraction
of all FC parameters, we can write $\phi^\prime = \phi - p \times
\phi_{\mathrm{fc}}$. We require two bytes per parameter for $\vec{\theta}_{16}$
and another two bytes per parameter for $\nabla\vec{\theta}_{16}$. Also, for
every parameter belonging to a pruned parameter tensor we require an additional
eight bytes to store the non-zero indices corresponding to the COO format.
Thus,
%
\begin{align}
    M^{\mathrm{PG}}_{\mathrm{gpu}} & = 2\phi^\prime + 2\phi^\prime + 8\phi_{\mathrm{fc}}(1-p) \\
    & = 4\phi^\prime + 4p\times\phi_{\mathrm{fc}} - 12p\times\phi_{\mathrm{fc}} + 8\phi_{\mathrm{fc}}\\
    & = 4\left( \phi^\prime + p\times\phi_{\mathrm{fc}} \right) - 4 \left( 3p-2 \right)\phi_{\mathrm{fc}} \\
    & = 4\phi - 4 \left( 3p-2 \right)\phi_{\mathrm{fc}}
\end{align}

Now, we will add the memory required to store the remaining tensors i.e.
$\vec{\theta}$, $\nabla\vec{\theta}$, and $\vec{s}_{\mathrm{opt}}$.
$\vec{\theta}$ and $\nabla\vec{\theta}$ are in single precision and therefore
each require four bytes per parameter. The Adam optimizer stores two state
variables in single precision for each parameter. Thus, we require eight bytes
per parameter for $\vec{s}_{\mathrm{opt}}$. Therefore, a total of $4+4+8=16$
bytes per parameter is enough to store these tensors on the GPU DRAM. Thus,
%
\begin{align} 
    M_{\mathrm{gpu}} & = M^{\mathrm{PG}}_{\mathrm{gpu}} + 16\phi^\prime \\ 
    & = 4\phi - 4 \left( 3p-2 \right)\phi_{\mathrm{fc}} + 16\left ( \phi - p \times \phi_{\mathrm{fc}} \right)  \\
    & = 20\phi - 4 \left( 7p-2 \right)\phi_{\mathrm{fc}} \label{eq:lth}
\end{align}
%

Without LTH pruning and any other memory optimizations, the total memory
required to store model states is $20\phi$ (substitute $p=0$ in Equation
\ref{eq:lth}).  Thus, an interesting corollary of this result is that the
minimum sparsity $p$ of the pruned parameter tensors required to save memory
over the case with no memory optimizations should be greater than
$\frac{2}{7}$. Below this sparsity, we would in-fact end up increasing memory
consumption! We note that this requirement is well below the levels of
sparsities induced by applying LTH-based pruning to a neural network.

We now derive the state memory consumption when \stod is used in conjunction
with \axonn's memory optimization. Their algorithm deletes $\nabla\vec{\theta}$
and offloads $\vec{\theta}$, and $\vec{s}_{\mathrm{opt}}$ to the CPU. They
allocate a small fixed GPU buffer to prefetch/materialize subsets of these
tensors at a time for the optimizer computation. Assuming,
$\delta_{\mathrm{\axonn}}$ to be the size of this buffer,
%
\begin{align}
    M^{\mathrm{\prime}}_{\mathrm{gpu}} & = M^{\mathrm{PG}}_{\mathrm{gpu}} + \delta_{\mathrm{\axonn}} \\ 
    & = 4\phi - 4(3p-2)\phi_{\mathrm{fc}} + \delta_{\mathrm{\axonn}} \\
    & \approx 4\phi - 4(3p-2)\phi_{\mathrm{fc}} \left(\because 4\phi \gg \delta_{\mathrm{\axonn}}\right) \label{eq:cpu-lth}
\end{align}

Again, to provide additional memory savings over \axonn's memory optimizations,
we require a minimum sparsity of $\frac{2}{3}$, a level which is easily
achievable by LTH.

